Architectural Exploration of Application-Specific Resonant SRAM Compute-in-Memory (rCiM)

While general-purpose computing follows Von Neumann's architecture, the data movement between memory and processor elements dictates the processor's performance. The evolving compute-in-memory (CiM) paradigm tackles this issue by facilitating simultaneous processing and storage within static random-access memory (SRAM) elements. Numerous design decisions taken at different levels of hierarchy affect the figure of merits (FoMs) of SRAM, such as power, performance, area, and yield. The absence of a rapid assessment mechanism for the impact of changes at different hierarchy levels on global FoMs poses a challenge to accurately evaluating innovative SRAM designs. This paper presents an automation tool designed to optimize the energy and latency of SRAM designs incorporating diverse implementation strategies for executing logic operations within the SRAM. The tool structure allows easy comparison across different array topologies and various design strategies to result in energy-efficient implementations. Our study involves a comprehensive comparison of over 6900+ distinct design implementation strategies for EPFL combinational benchmark circuits on the energy-recycling resonant compute-in-memory (rCiM) architecture designed using TSMC 28 nm technology. When provided with a combinational circuit, the tool aims to generate an energy-efficient implementation strategy tailored to the specified input memory and latency constraints. The tool reduces 80.9% of energy consumption on average across all benchmarks while using the six-topology implementation compared to baseline implementation of single-macro topology by considering the parallel processing capability of rCiM cache size ranging from 4KB to 192KB.

==> coverletter.tex <==



\signature{Dhandeep Challagundla\\Ignatius Bezzam\\Riadul Islam} % name for signature 
\longindentation=0pt    % needed to get closing flush left
\let\raggedleft\raggedright     % needed to get date flush left
 
\begin{letter}
{} 
\vspace{-4.5cm}
 
\opening{Dear Transactions on Very Large Scale Integration (VLSI) Reviewers:} 

\noindent We would like to thank all of you you for reviewing the paper, and the opportunity to resubmit a revised copy of the manuscript. We would like to take this opportunity to express our thanks to the reviewers for the positive feedback and helpful comments for corrections and modifications. The manuscript has been revised to address the reviewer's comments, and a separate document with responses to the reviewer's feedback has been included alongside this document.

\noindent Below is the summary of changes made to the manuscript:

\begin{enumerate}
 \setlength{\itemsep}{1pt}
 \setlength{\parskip}{0pt}
 \setlength{\parsep}{0pt}

        \item The main contributions section has been updated to provide a clearer summary of the key innovations of the work.
        \item Figure 4 has been revised to include the structure of the Sense Amplifier (SA) along with the corresponding discharge times for NAND2 and NOR2 operations.
        \item Figure 7 has been enhanced to show an example of the mapping strategy for both single-macro and three-macro implementations.
        \item The algorithm has been clarified with improved descriptions for the parts that were previously confusing, as mentioned by the reviewers.
        \item Additional clarification on the total power consumption across different macro implementations is provided for the Figure 9.
        \item A process variation analysis for the sense amplifier has been added to ensure completeness of the work.
        \item The comparison of this work with other State-of-the-Art designs has been updated.
 \end{enumerate}


   

\closing{Sincerely,}

\end{letter}


